Strategy Derivation for Small Progress Measures

Small Progress Measures is one of the most efficient parity game solving algorithms. The original algorithm provides the full solution (winning regions and strategies) in $O(dm \cdot (n/\lceil d / 2 \rceil)^{\lceil d/2 \rceil})$ time, and requires a re-run of the algorithm on one of the winning regions. We provide a novel operational interpretation of progress measures, and modify the algorithm so that it derives the winning strategies for both players in one pass. This reduces the upper bound on strategy derivation for SPM to $O(dm \cdot (n/\lfloor d / 2 \rfloor)^{\lfloor d/2 \rfloor})$.

==> algorithm-backup.tex <==
\begin{algorithm}[h!t]
\caption{Modified SPM with strategy derivation for player Odd}
\label{alg:newspm}
%\scriptsize
\begin{algorithmic}[1]
\Function{Solve}{$G$}
\State \emph{\textbf{Input} $G = (V, E, \priosym, (V_\even, V_\odd))$}
\State \emph{\textbf{Output} Winning partition and strategies $((W_\even,\sigma'),(W_\odd,\sigma))$}
%\State \Comment{$G$ is of the form $(V,E, \priosym,(V_\even,V_\odd))$}
\State initialise $\sigma$ to an empty assignment
\State $\rho \gets \Call{NewSPM}{G}$
%\State $W_{\odd} \gets \{w \,\mid\, \rho(w) = \top \}$
%\State $W_{\even} \gets V \setminus W_{\odd}$
\State compute strategy $\sigma'$ for player Even by picking min. successor w.r.t. $\rho$
%\State \Return $((W_{\even},\sigma'),(W_{\odd},\sigma))$
\State \Return $((\{v \in V ~|~ \rho(v) \neq \top\},\sigma'),(\{v \in V ~|~ \rho(v) = \top,\sigma))$

\State

\Function{NewSPM}{$G$}  
\State \emph{\textbf{Input} $G = (V, E, \priosym, (V_\even, V_\odd))$}
\State \emph{\textbf{Output} Least game parity progress measure $\rho$}
%\State \Comment{Computes the smallest progress measure for game $G \cap V$.}
%\State \Comment{Upon termination $\rho$ is assigned the smallest progress measure for $G$ and}
%\State \Comment{for every vertex $w $ with $\rho(w) = \top$, the local strategy $\sigma$ is assigned.}
\State $\rho  \gets \lambda w \in V.~(0, \dots, 0)$
\While{$(G \neq \text{empty game})$}
\While{$\rho \sqsubset \lift{\rho}{w} \text{for some $w \in V$ and for all $w \in V$:} \rho(w) \neq \top$} \label{line:liftloop_start}
\State $\rho \gets \lift{\rho}{w}$ for $w \in V$ such that $\rho \sqsubset \lift{\rho}{w}$
\EndWhile \label{line:liftloop_end}
\State \textbf{if} {$\text{for all $w \in V$: } \rho(w) \neq \top$} \textbf{return} $\rho$ \textbf{end if}

\State $v \gets $ the only vertex such that $\rho(v) = \top$
\State $k \gets \prio{v}$
\State \label{line:firsttop_strat} $\sigma(v) \gets u$ where $u \in v^\bullet$ for which $\rho(u') \leq_{k} \rho(u)$ for all $u' \in v^\bullet$
\State $\res \gets \myattr{\geq k}{\odd}{\{v\}}$
\For{ \textbf{all} $w \in \res \setminus \{v\}$}
\State $\rho(w) \gets \top$
\If{$w \in V_{\odd}$} assign $\sigma(w)$ to be the strategy \emph{attracting} to $v$
\EndIf 
\EndFor \label{line:defsigma_res_end}
\State $\dom \gets \res$
\If{$\sigma$ is not closed on $\dom$}
  \State $\irr \gets \attr{\even}{\{ w \in V \,\mid\, \prio{w} < k\}}$
  \State \label{line:rem} $\rem \gets V \setminus (\res \cup \irr)$
  \State \label{line:reccall} $\rho' \gets \Call{NewSPM}{G \cap \rem}$  
  \State $\dom \gets \dom \cup \{ w \in \rem \,\mid\, \rho'(w) = \top \}$ \label{line:dominion_resolved}
  \State \textbf{for all} $w \in \rem: \rho'(w) = \top$ \textbf{do} $\rho(w) \gets \top $ \textbf{end for}
\EndIf
\State $A \gets \attr{\odd}{\dom}$

  \For{ \textbf{all} $w \in A \setminus \dom$}
  \State $\rho(w) \gets \top$
    \If{$w \in V_{\odd}$} 
    assign $\sigma(w)$ to be the strategy  \emph{attracting} to $\dom$ 
    \EndIf
  \EndFor
\State $G \gets G \setminus A$
\EndWhile
\State \Return $\rho$
%\State \Return $(W_\even, W_\odd)$
\EndFunction
\EndFunction

\end{algorithmic}
\end{algorithm}



==> algorithm.tex <==
\begin{algorithm}[h!t]
\caption{Modified SPM with strategy derivation for player Odd}
\label{alg:newspm}
%\scriptsize
\begin{algorithmic}[1]
\State Assume a global variable $\sigma$, initialised to an empty assignment and a game $G = (V,E, \priosym,(V_\even,V_\odd))$

\Function{NewSPM}{$G$}  
%\State \Comment{Computes the smallest progress measure for game $G \cap W$.}
%\State \Comment{Upon termination $\rho$ is assigned the smallest progress measure for $G$ and}
%\State \Comment{for every vertex $w $ with $\rho(w) = \top$, the local strategy $\sigma$ is assigned.}
\State initialise $\rho$ to $0$-tuples
\While{$(W \neq \emptyset)$}
\While{for some $v \in W$: $\rho \sqsubset \lift{\rho}{v} \wedge \text{for all $w \in W$:} \rho(w) \neq \top$} \label{line:liftloop_start}
\State $\rho \gets \lift{\rho}{v}$ for $v \in W$ such that $\rho \sqsubset \lift{\rho}{v}$
\EndWhile \label{line:liftloop_end}
\If{$\text{for all $w \in W$: } \rho(w) \neq \top$} 
\State \textbf{break}
\EndIf
\State $v \gets $ the only vertex in $W$ such that $\rho(v) = \top$
\State $k \gets \prio{v}$
\State \label{line:firsttop_strat} $\sigma(v) \gets u$ where $u \in W \cap v^\bullet$ for which $\rho(u') \leq_{\prio{v}} \rho(u)$ for all $u' \in v^\bullet \cap W$
\State $\res \gets \myattrW{\geq k}{\odd}{\{v\}}{W}$
\For{ \textbf{all} $w \in \res \setminus \{v\}$}
\State $\rho(w) \gets \top$
\If{$w \in V_{\odd}$} assign $\sigma(w)$ to be the strategy \emph{attracting} to $v$
\EndIf
\EndFor%\textbf{end for}

\If{$\sigma$ is closed on $\res$}
  \State $\dom \gets \res$
\Else
  \State $\irr \gets \myattrW{}{\even}{\{ w \in W \,\mid\, \prio{w} < k\}}{W}$
  \State \label{line:reccall} $\Call{NewSPM}{W \setminus (\res \cup \irr)}$  
  \State $\dom \gets \res \cup \{ w \in W \,\mid\, \rho'(w) = \top \}$ \label{line:dominion_resolved}
\EndIf
\State $A \gets \myattrW{}{\odd}{\dom}{W}$

  \For{ \textbf{all} $w \in A \setminus \dom$}
  \State $\rho(w) \gets \top$
    \If{$w \in V_{\odd}$} 
    assign $\sigma(w)$ to be the strategy  \emph{attracting} to $\dom$ 
    \EndIf
  \EndFor
\State $W \gets W \setminus A$
\EndWhile
%\State \Return $(W_\even, W_\odd)$

\If{$W = V$}
\State $W_{\odd} \gets \{w \,\mid\, \rho(w) = \top \}$
\State $W_{\even} \gets V \setminus W_{\odd}$
\State compute strategy $\sigma'$ for player \even by picking the min. successor w.r.t. $\rho$
\State \Return $((W_{\even},\sigma'),(W_{\odd},\sigma))$
\EndIf
\EndFunction

\end{algorithmic}
\end{algorithm}



==> old_algorithm.tex <==
\begin{algorithm}[ht]
\caption{Modified SPM with strategy derivation for player Odd}
\label{alg:newspm}
%\scriptsize
\begin{algorithmic}[1]
\State Assume global variables $\varrho$ and $\sigma$.

\Function{Solve}{$G$}
\State initialise $\varrho$ to $0$-tuples and $\sigma$ to an empty assignment
\State $\Call{NewSPM}{G}$
\State compute strategy $\sigma'$ for player Even in a standard way (picking min. successor w.r.t. $\varrho$)
\State return the winning sets and the corresponding strategies
\EndFunction

\Function{NewSPM}{$G$}  
\State \Comment{Computes the smallest progress measure for (sub)game $G$.}
\State \Comment{Upon termination $\varrho$ is assigned the smallest progress measure for $G$ and}
\State \Comment{for every vertex $w $ with $\rho(w) = \top$, the local strategy $\sigma$ is assigned.}
\While{$(G \neq \emptyset)$}

\State \textbf{while} $($\text{for all $w \in G$ } $\rho(w) \neq \top ) \wedge (\varrho$ \text{ is not stable}$))$ \text{lift } $\rho$ \textbf{end while}
\State \textbf{if} $(\varrho$ \text{is stable}$)$ \Return \textbf{end if}

\State $v \gets $ the only vertex in G such that $\varrho(v) = \top$; $k \gets \prio{v}$
\State $\sigma(v) \gets$ successor of $v$ with max. $\varrho$
\State $B = \myattr{\geq k}{\odd}{\{v\}}$
\For{ \textbf{all} $w \in (B \setminus \{v\})$}
\State $\varrho(w) \gets \top$
\State \textbf{if} ($w \in V_{\odd}$) assign $\sigma(w)$ to be the strategy  ``attracting'' to $v$ \textbf{end if}
\EndFor%\textbf{end for}
\State $U = \attr{\even}{\{ w \,\mid\, \prio{w} < k\}}$
\State $G' = G \setminus(B \cup U)$
\State $\Call{NewSPM}{G'}$
\State $B' = B \cup \{ w \in G' \,\mid\, \varrho(w) = \top \}$

\For{ \textbf{all} $w \in (\attr{\odd}{B'} \setminus B')$}
\State $\varrho(w) \gets \top$
\State \textbf{if} ($w \in V_{\odd}$) assign $\sigma(w)$ to be the strategy  ``attracting'' to $B'$ \textbf{end if}
\EndFor
\State $G \gets G \setminus \attr{\odd}{B'} $
\EndWhile
%\State \Return $(W_\even, W_\odd)$
\EndFunction

\end{algorithmic}
\end{algorithm}


==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

We briefly introduce parity games in Section~\ref{sec:parity_games} and
Jurdzi\'nski's Small Progress Measures algorithm in Section~\ref{sec:spm}.
For an in-depth treatment of both, we refer to~\cite{2001automata} and the
references therein.

\subsection{Parity Games}
\label{sec:parity_games}
A parity game is an infinite duration game, played by players \emph{odd},
denoted by $\odd$ and \emph{even}, denoted by $\even$, on a directed,
finite graph. The game is formally defined as follows.

\begin{definition}
A parity game is a tuple $(V, E, \priosym, (V_\even,V_\odd))$, where
\begin{itemize}
\item $V$ is a finite set of vertices, partitioned in a set $V_\even$ of
vertices owned by player $\even$, and a set of vertices $V_\odd$ 
owned by player $\odd$,
\item $E \subseteq V \times V$ is a total edge relation,
\item $\priosym \oftype V \to \nat$ is a priority function that assigns
priorities to vertices.
\end{itemize}
\end{definition}
Parity games are depicted as graphs; diamond-shaped nodes
represent vertices owned by player $\even$, box-shaped nodes
represent vertices owned by player $\odd$ and the priority assigned
to a vertex is written inside the node.

Throughout this section, assume that $G = (V,E,\priosym, (V_\even,
V_\odd))$ is an arbitrary parity game.  We write $v \to w$ iff
$(v,w) \in E$, and $\post{v}$ to denote the set of successors of
$v$, \ie\ $\{w \in V ~|~ v \to w\}$.  Moreover, $V_i = \{ v \in V
\mid \priosym(v) = i \}$ and $V_{\le k}$ and $V_{\ge k}$ are defined
similarly.  Henceforth, we assume that $\i$ denotes
an arbitrary player; that is $\i \in \{\odd,\even\}$. We write
$\pnot{\i}$ for $\i$'s opponent:  $\pnot{\even}=\odd$ and
$\pnot{\odd}=\even$.  For a set $A \subseteq V$, we define $G \cap
A$ as the structure $(A, E \cap (A \times A), \priosym|_A, (V_\even
\cap A, V_\odd \cap A))$; the structure $G \setminus A$ is defined
as $G \cap (V \setminus A)$. The structures $G \cap A$ and $G \setminus A$ are
again a parity game if their edge relations are total; in general, this is not the
case.

We will now define an attractor, which, intuitively, captures the phenomenon of forced reachability. An $\i$-\emph{attractor} into a set $U \subseteq V$ contains vertices, from which player $\i$ can force any play to $U$.
%
\begin{definition} The $\i$-\emph{attractor} into a set $U \subseteq V$,
denoted $\attr{\i}{U}$, is the least set $A \subseteq V$ satisfying:
\begin{enumerate}
 \item $U \subseteq A$
 \item
 \begin{enumerate}
 \item if $w \in V_{\i}$ and $\post{w} \cap A \neq \emptyset$, then $w \in A$
 \item if $w \in V_{\pnot{\i}}$ and $\post{w} \subseteq A$, then $w \in A$
 \end{enumerate}
\end{enumerate}

\end{definition}

Observe that the complement of an attractor set of any subset of a parity game induces a parity game, i.e. $G  \setminus \attr{\i}{U}$ for any $U$ and $\i$ is a well-defined parity game.

\paragraph{Plays and Strategies}
A sequence of vertices $v_1, \ldots, v_n$ is a \emph{path} if $v_m \to
v_{m+1}$ for all $1 \leq m < n$.  Infinite paths are defined in a similar
manner. We write $p_i$ to denote the $i^\textrm{th}$ vertex in a path $p$.

A game starts by placing a token on some vertex $v \in V$.  Players
$\even$ and $\odd$ move the token indefinitely according to a single
simple rule: if the token is on some vertex that belongs to player
$\i$, that player moves the token to an adjacent vertex.
An infinite sequence of vertices created this way is called a
\emph{play}.  The \emph{parity} of the \emph{least} priority that occurs
infinitely often on a play defines the \emph{winner} of the play:
player $\even$ wins if, and only if this priority is even. This is
known as the \emph{parity condition}.  Note that, alternatively,
one could demand that the \emph{highest} priority that occurs
infinitely often along a play determines the winner; such games
would be \emph{max} parity games. 

%%
%% Strategies
%%

A \emph{strategy} for player $\i$ is a partial function $\sigma
\oftype V^+ \to V$ satisfying that whenever it is defined for a finite 
path $u_1 \cdots u_n \in V^+$, both $u_n \in
V_{\i}$ and $\sigma(u_1\cdots u_n) \in \post{u_n}$. 
An infinite play $u_1\ u_2\ u_3 \cdots$ is \emph{consistent} with a strategy 
$\sigma$ if all prefixes $u_1 \cdots u_n$ of the play
for which $\sigma(u_1\ \cdots u_n)$ is defined, $u_{n+1} =
\sigma(u_1 \cdots u_n)$.   

Some strategy $\sigma$ is winning for player $\i$ from vertex $v$
iff all plays consistent with $\sigma$ are won by player $\i$.
Vertex $v$ is won by player $\i$ whenever she has a winning strategy
for all plays starting in vertex $v$.  Remark that parity games are
\emph{determined}~\cite{EJ:91}, meaning that every vertex is won
by one of the players; they are even \emph{positionally determined},
meaning that if $\i$ wins a vertex then she has a winning
\emph{positional strategy}: a strategy that determines where to
move the token next based solely on the vertex on which the token
currently resides. Such strategies can be represented by a function
$\sigma\oftype V_{\i} \to V$.  Whenever we refer to an \emph{attractor
strategy} associated with $\attr{\i}{U}$, we mean the positional
strategy that player $\i$ can employ to force play to $U$; such a
strategy can be computed in $\mathcal{O}(|V|+|E|)$ using a
straightforward fixpoint iteration.

\emph{Solving} a parity game $G$ essentially means computing the partition
$(\winsubeven{G},\winsubodd{G})$ of $V$ into vertices won by player $\even$ and
player $\odd$, respectively.  

A set of vertices $U$ is an
$\i$-dominion whenever there is a strategy $\sigma$ for player $\i$ such that every play starting in $U$ and conforming to $\sigma$ is winning for $\i$ and stays within $U$. A game is a \emph{paradise} for player $\i$ if the entire game is an
$\i$-dominion.

We shall frequently work with strategies or dominions \emph{in the context of a certain subgame $G' \subset G$}, which do not retain their properties when moving to a larger context of $G$. For instance, consider a subset of vertices $W \subset V$ that induces a subgame $G \cap W$, and moreover that there is a subset $D \subseteq W$ which is a \player-dominion \emph{in $G \cap W$}. Observe that, in general, $D$ is not a \player-dominion within $G$. In such cases we always explicitly state which context is assumed.

For a set of vertices $W \subseteq V$, we will denote the minimal priority occurring in $W$ with $\minprio{W}$.

Given a finite or infinite play $\pi$, a \emph{stretch} is a finite subsequence of $\pi$, $\pi_s \pi_{s+1} \dots \pi_{s+l}$. For a priority $k$, a \emph{$k$-dominated stretch} is a stretch in which the minimal priority among all vertices in the stretch is $k$.


%$U$ is $\i$-closed ($\i$ can force the
%play to remain within $U$) and the induced subgame is won by $\i$;




==> section3.tex <==

\newcommand{\Nat}{\ensuremath{\mathbb{N}}}
\newcommand{\prog}[3]{\ensuremath{\textsf{Prog}(#1,#2,#3)}}
\newcommand{\lift}[2]{\ensuremath{\textsf{Lift}(#1,#2)}}
\newcommand{\liftodd}[2]{\ensuremath{\textsf{Lift}_\odd(#1,#2)}}
\def\progname{\textsf{Prog}}
\def\liftname{\textsf{Lift}}




\subsection{Jurdzi\'nski's Small Progress Measures Algorithm}
\label{sec:spm}
\myomit{\mycomment{change}
Jurdzi\'nski's essential insight that ultimately led to the small
progress measures (SPM) algorithm  was that deciding the winners in
a parity game can be done by characterising the cycles, reachable
from each vertex. For instance, player $\even$ wins a vertex iff she can
force play such that all cycles appearing in the play are even. }
The SPM algorithm works by computing a \emph{measure} associated with
each vertex that characterises even (resp.\ odd) cycles: it is such
that it decreases along the play with each ``bad'' odd priority
encountered, and only increases upon reaching a beneficial even
priority. In what follows, we recapitulate the essentials for defining
and studying the SPM algorithm; our presentation is---as in
the original paper by Jurdzi\'nski---from the perspective of player
$\even$. \medskip

Let $G = (V, E, \priosym, (V_{\even}, V_{\odd}))$ be a parity game.
Let $d$ be a positive number and let $\alpha
\in \Nat^d$ be a \emph{$d$-tuple} of natural numbers.  We number
its components from $0$ to $d-1$, \ie $\alpha = (\alpha_0, \alpha_1,
\dots, \alpha_{d-1})$, and let $<$ on such $d$-tuples be given by
the lexicographic ordering. These tuples will be used to (partially)
record how often we can or must see vertices of a particular priority
on all plays. We define a derived ordering $<_i$ on $k$-tuples and
$l$-tuples of natural numbers as follows:
\[
(\alpha_0, \alpha_1, \dots, \alpha_k) <_i (\beta_0,\beta_1,\dots,\beta_l)
\text{ iff }
(\alpha_0, \alpha_1, \dots, \alpha_i) < (\beta_0,\beta_1,\dots,\beta_i)
\]
where, if $i > k$ or $i >l$, the tuples are suffixed with $0$s.
Analogously, we write $\alpha =_i \beta$ to denote that $\alpha$ and
$\beta$ are identical up-to and including position $i$.
Intuitively, the derived ordering provides enough information to
reason about the interesting bits of plays: when encountering a
priority $i$ in a play, we are only interested in how often we can
or must visit vertices of a more significant (\ie smaller) priority
than $i$, whereas we no longer care about how often we have seen
less significant priorities.

Now, assume from hereon that $d-1$ is the largest priority occurring in
$G$; \ie, $d$ is one larger than the largest priority
in $G$.  For $i \in \Nat$, let $n_i = |V_i|$. 
Define $\mathbb{M}^{\even} \subseteq \Nat^d \cup \{\top\}$, containing $\top$
($\top \notin \Nat^d$)
and only those $d$-tuples with $0$ on \emph{even} positions and
natural numbers $\leq$ $n_i$ on \emph{odd} positions $i$.

The lexicographical ordering $<$ and the family of orderings
$<_i$ on $d$-tuples is extended to an ordering on $\mathbb{M}^\even$
by setting $\alpha < \top$ and $\top = \top$. 
Let $\rho {:} V \to \mathbb{M}^\even$ and suppose $w \in \post{v}$. Then
$\prog{\rho}{v}{w}$ is the least $m \in \mathbb{M}^{\even}$, such that
\begin{itemize}
  \item $m \geq_{\prio{v}} \rho(w)$ if $\prio{v}$ is even,
  \item $m >_{\prio{v}} \rho(w)$, or $m = \rho(w) = \top$ if $\prio{v}$ is odd.
\end{itemize}
\begin{definition} Function
$\rho$ is a \emph{game parity progress measure}
if for all $v \in V$:
\begin{itemize}
  \item if $v \in V_{\even}$, then for some $w \in \post{v}$, $\rho(v) \geq_{\prio{v}} \prog{\rho}{v}{w}$
  \item if $v \in V_{\odd}$, then for all $w \in \post{v}$, $\rho(v) \geq_{\prio{v}}\prog{\rho}{v}{w}$
\end{itemize}
\end{definition}



\begin{proposition}[Jurdzi\'nski~\cite{Jur:00}]\label{prop:jurdzinski}
If $\rho$ is the \emph{least} game parity progress measure, then for all $v \in V$:
$\rho(v) \neq \top$ iff $v \in W_{\even}$.
\end{proposition}
The least game parity progress measure can be characterised as the least fixpoint
of a monotone transformer on the complete lattice we define next. Let
$\rho,\rho' {:} V \to \mathbb{M}^\even$ and define
$\rho \sqsubseteq \rho'$ as $\rho(v) \leq \rho'(v)$ for all $v \in V$. We write
$\rho \sqsubset \rho'$ if $\rho \sqsubseteq \rho'$ and $\rho \not= \rho'$. Then
the set of all functions $V \to \mathbb{M}^\even$ with $\sqsubseteq$ is a complete
lattice. The monotone transformer defined on this set is given as follows:
\[
\lift{\rho}{v} = \begin{cases}
\rho[v \mapsto \min\{ \prog{\rho}{v}{w} \mid v \to w \}] &
\text{if $v \in V_{\even}$}\\
\rho[v \mapsto \max\{ \prog{\rho}{v}{w} \mid v \to w \}] &
\text{if $v \in V_{\odd}$}
\end{cases}
\]
As a consequence of Tarski's fixpoint theorem, we know the least fixpoint of the
above monotone transformer exists and can be computed using Knaster-Tarski's iteration
scheme. This leads to the original SPM algorithm, see Algorithm~\ref{alg:spm}.
\begin{algorithm}[h!]
\begin{algorithmic}[1]
\Function{SPM}{$G$}
\State \emph{\textbf{Input} $G = (V, E, \priosym, (V_\even, V_\odd))$}
\State \emph{\textbf{Output} Winning partition $(\winsubeven{G},\winsubodd{G})$}
\State $\rho  \gets \lambda v \in V.~(0, \dots, 0)$
\While{$\rho \sqsubset \lift{\rho}{v}$ for some $v \in V$}
  \State $\rho \gets \lift{\rho}{v}$ for some $v \in V$ such that $\rho \sqsubset \lift{\rho}{v}$
\EndWhile
\State \Return $(\{v \in V ~|~ \rho(v) \not= \top\}, \{v \in V ~|~ \rho(v) = \top\})$
\EndFunction
\end{algorithmic}
\caption{The original Small Progress Measures Algorithm}
\label{alg:spm}
\end{algorithm}
Upon termination of the iteration within the SPM algorithm, the
computed game parity progress measure $\rho$ is used to compute the
sets $\winsubeven{G}$ and $\winsubodd{G}$ of vertices won by player $\even$ and
$\odd$, respectively.  Moreover, a memoryless winning strategy
$\sigma_\even {:} V_\even \to V$ for player $\even$ can be extracted
from $\rho$ by setting $\sigma_\even(v) = w$ for $v \in V_\even
\cap \winsubeven{G}$ and $w \in \post{v}$ such that $\rho(w) \le \rho(w')$
for all $w' \in \post{v}$.  A winning strategy for player $\odd$
cannot be extracted from $\rho$ \emph{a posteriori}. The community
solution to this problem is to solve the game again, but now from
the perspective of player $\odd$, or to simultaneously solve the
game for both players; see~\eg~\cite{FL:14}.

To facilitate the analysis of SPM, we will introduce certain additional terms and notions. 

\def\liftseq{ms}

A convenient abstraction of an instance of SPM being executed on a particular game is a sequence of intermediate measure values $\rho_0 \rho_1 \dots \rho_C$, where $\rho_C$ is the current measure value (as we frequently consider partial executions of SPM, $\rho_C$ is not necessarily the final, stable measure). Formally, we define a \emph{lifting context} as a tuple $\tuple{G,\liftseq}$, where $G$ is a parity game, and 
$\liftseq = \rho_0 \rho_1 \dots \rho_C$ a sequence of all intermediate measure values.

Note that we use the term \emph{measure} to refer to the intermediate values of $\rho$ as well.

Given a tuple $m \in \mathbb{M}^\even$, we say that the position $i$ in $m$ is \emph{saturated}, if $(m)_i = |V_i|$.



==> section4.tex <==

\section{An Enhanced Small Progress Measures Algorithm}

A basic enhancement of the Small Progress Measures algorithm is to
solve a parity game using both the even and odd measures
$\mathbb{M}^\even$ and $\mathbb{M}^\odd$ at the same time, and
returning the solved game as soon as one of the computations has
yielded a stable game parity progress measure. Moreover,
the running time of the algorithm can be expected to benefit from
integrating it with an SCC decomposition, leading to 
Algorithm~\ref{alg:spm_enhanced}. Note that the correctness of the
algorithm follows essentially again from Proposition~\ref{prop:jurdzinski}.
\begin{algorithm}[h!]
\begin{algorithmic}
\Function{ESPM}{$G$}
\State \emph{\textbf{Input} $G = (V, E, \priosym, (V_\even, V_\odd))$}
\State \emph{\textbf{Output} Winning partition $(W_\even, W_\odd)$}

\State $W_\even, W_\odd \gets \emptyset,\emptyset$
\State $\mathcal{S} \gets \{C \subseteq V ~|~ C \text{ is an SCC } \}$
\While{$\mathcal{S} \not= \emptyset$}
\State $C \gets $ bottom SCC in $\mathcal{S}$
\State $(A_\even,A_\odd) \gets \Call{Solve}{G \cap C}$
\State $(W_\even, W_\odd) \gets (W_\even \cup \attr{\even}{ A_\even }, 
                W_\odd \cup \attr{\odd}{ A_\odd })$
\State $\mathcal{S} \gets \{C \subseteq V \setminus (W_\even \cup W_\odd) ~|~ C \text{ is an SCC } \}$
\EndWhile
\State \Return $(W_\even,W_\odd)$
\EndFunction
\State

\Function{Solve}{$G$}
\State \emph{\textbf{Input} $G = (V, E, \priosym, (V_\even, V_\odd))$}
\State \emph{\textbf{Output} Winning partition $(W_\even, W_\odd)$}
\State $\rho  \gets \lambda v \in V.~(0, \dots, 0)$
\State $\rho_\Box  \gets \lambda v \in V.~(0, \dots, 0)$
\While{$\rho \sqsubset \lift{\rho}{v}$ and $\rho_\Box \sqsubset \liftodd{\rho_\Box}{u}$ 
for some $u,v \in V$}
  \State $\rho \gets \lift{\rho}{v}$ for some $v \in V$ such that $\rho \sqsubset \lift{\rho}{v}$
  \State $\rho_\Box \gets \liftodd{\rho_\Box}{u}$ for some $u \in V$ such that $\rho_\Box \sqsubset \liftodd{\rho_\Box}{u}$
\EndWhile
\If{$\rho = \lift{\rho}{v}$ for all $v \in V$}
\Return $(\{v \in V ~|~ \rho(v) \not= \top\}, \{v \in V ~|~ \rho(v) = \top \} ) $
\Else{}
\Return $(\{v \in V ~|~ \rho_\Box(v) = \top\}, \{v \in V ~|~ \rho_\Box(v) \not= \top \} ) $
\EndIf
\EndFunction
\end{algorithmic}
\caption{An Enhanced Small Progress Measures Algorithm.
}
\label{alg:spm_enhanced}
\end{algorithm}

\paragraph{Solving Weak Games}

\begin{theorem}
Algorithm~\ref{alg:spm_enhanced} solves weak games in polynomial time.
\end{theorem}

\paragraph{Solving Dull Games}

\begin{theorem}
Algorithm~\ref{alg:spm_enhanced} solves dull games in polynomial time.
\end{theorem}

\paragraph{Solving Solitaire Games}

Contrary to the above game classes, Algorithm~\ref{alg:spm_enhanced} cannot
solve these games in polynomial time. While the solitaire game we used in the
previous section to show that the Algorithm~\ref{alg:spm} requires exponential time
on solitaire games now can be solved in polynomial time, the solitaire game depicted
in Figure~\ref{fig:solitaire3} still requires exponential time.

\begin{theorem}
Algorithm~\ref{alg:spm_enhanced} requires exponential time to solve solitaire games.
\end{theorem}
\input{solitaire3}



